Residual Neural Networks for Digital Predistortion

Tracking the nonlinear behavior of an RF power amplifier (PA) is challenging. To tackle this problem, we build a connection between residual learning and the PA nonlinearity, and propose a novel residual neural network structure, referred to as the residual real-valued time-delay neural network (R2TDNN). Instead of learning the whole behavior of the PA, the R2TDNN focuses on learning its nonlinear behavior by adding identity shortcut connections between the input and output layer. In particular, we apply the R2TDNN to digital predistortion and measure experimental results on a real PA. Compared with neural networks recently proposed by Liu et al. and Wang et al., the R2TDNN achieves the best linearization performance in terms of normalized mean square error and adjacent channel power ratio with less or similar computational complexity. Furthermore, the R2TDNN exhibits significantly faster training speed and lower training error.

==> Figures/acpr_vs_flops.tex <==
\begin{tikzpicture}[scale=\linewidth/14cm]
\definecolor{mycolor1}{rgb}{0.12156862745098039, 0.4666666666666667, 0.7058823529411765}%
\definecolor{mycolor2}{rgb}{1.0, 0.4980392156862745, 0.054901960784313725}%
\definecolor{mycolor3}{rgb}{0.17254901960784313, 0.6274509803921569, 0.17254901960784313}%
\definecolor{mycolor4}{rgb}{0.8392156862745098, 0.15294117647058825, 0.1568627450980392}%
\definecolor{mycolor5}{rgb}{0.5803921568627451, 0.403921568627451, 0.7411764705882353}%
\definecolor{mycolor6}{rgb}{0.5490196078431373, 0.33725490196078434, 0.29411764705882354}%
\definecolor{mycolor7}{rgb}{0.8901960784313725, 0.4666666666666667, 0.7607843137254902}%
\definecolor{mycolor8}{rgb}{0.4980392156862745, 0.4980392156862745, 0.4980392156862745}%
\definecolor{mycolor9}{rgb}{0.7372549019607844, 0.7411764705882353, 0.13333333333333333}%
\definecolor{mycolor10}{rgb}{0.09019607843137255, 0.7450980392156863, 0.8117647058823529}%

\begin{axis}[%
width=12cm,
height=9cm,
at={(2.19in,0.9in)},
scale only axis,
legend cell align={left},
legend style={at={(1,1)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black, font=\small},
log basis x={10},
tick align=outside,
tick pos=left,
 grid style={white!69.0196078431373!black},
xlabel style={font=\color{white!15!black}},
xlabel={Number of FLOPs},
xmajorgrids,
xmin=44, xmax=16008,
xminorgrids,
xmode=log,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel style={font=\color{white!15!black}},
ylabel={ACPR (dBc)},
ymajorgrids,
ymin=-50.8319688683529, ymax=-34.7286537645897,
yminorgrids,
ytick style={color=black}
]
% GMP-markers
\addplot [color=mycolor1, only marks, line width=2.0pt, mark=o, mark options={solid, color=mycolor1, scale=1.25}, forget plot]
table{%
44 -35.5388866454343
62 -37.4043635698105
94 -38.6845638003273
188 -42.4970017787448
284 -42.8223039934716
514 -43.1292782072731
744 -43.0719167514693
1916 -42.8158289631368
};
%GMP line
\addplot [color=mycolor1, solid, line width=2.0pt]
table{%
44 -35.5388866454343
62 -37.4043635698105
94 -38.6845638003273
188 -42.4970017787448
284 -42.8223039934716
514 -43.1292782072731
744 -43.0719167514693
1916 -42.8158289631368
};
\addlegendentry{GMP~\cite{GMP_2006}}


% RVTDNN-1, markers
\addplot [color=mycolor2, only marks, line width=2.0pt, mark=square, mark options={solid, mycolor2, scale=1.25}, forget plot]
table {%
60 -35.4863066
140 -36.00582274
220 -36.53884986
440 -39.06522179
880 -41.56616586
1760 -44.3708277
3480 -46.36154476
6980 -46.93934852
14000 -47.3680943
};
% RVTDNN-1 line
\addplot [color= mycolor2, dashed, line width=2.0pt]
table {%
60 -35.4863066
140 -36.00582274
220 -36.53884986
440 -39.06522179
880 -41.56616586
1760 -44.3708277
3480 -46.36154476
6980 -46.93934852
14000 -47.3680943
};
\addlegendentry{$K=3$, RVTDNN~\cite{liu2004dynamic}}

% ARVTDNN-1, markers
\addplot [color=mycolor4, only marks, line width=2.0pt, mark=triangle, mark options={solid, mycolor4, scale=1.25}, forget plot]
table {%
132 -36.23261020749107
220 -37.17557482673871
440 -38.50535113057343
968 -40.70538303738968
1936 -43.22064359425523
3872 -45.75602089720375
7656 -46.93483480552989
15356 -47.07963807421149
%30800 -47.00622906362934
};
% ARVTDNN-1 line
\addplot [color= mycolor4, dashed, line width=2.0pt]
table {%
132 -36.23261020749107
220 -37.17557482673871
440 -38.50535113057343
968 -40.70538303738968
1936 -43.22064359425523
3872 -45.75602089720375
7656 -46.93483480552989
15356 -47.07963807421149
%30800 -47.00622906362934
};
\addlegendentry{$K=3$, ARVTDNN~\cite{wang2018augmented}}

% R2TDNN-1, markers
\addplot [color=mycolor3, only marks, line width=2.0pt, mark=x, mark options={solid, mycolor3, scale = 1.75}, forget plot]
table {%
62 -35.46062263
142 -36.77988383
222 -37.91548916
442 -39.34902855
882 -42.15034333
1762 -45.03385619
3482 -46.38768519
6982 -47.43935367
14002 -47.47315317
};
% R2TDNN-1, line
\addplot [color=mycolor3, dashed, line width=2.0pt]
table {%
62 -35.46062263
142 -36.77988383
222 -37.91548916
442 -39.34902855
882 -42.15034333
1762 -45.03385619
3482 -46.38768519
6982 -47.43935367
14002 -47.47315317
};
\addlegendentry{$K=3$, R2TDNN}

% % RVTDNN-2, markers
% \addplot [color=mycolor2, mark=square,line width=2.0pt, only marks, mark options={solid, scale=1.25}, forget plot]
% table {%
% 48 -35.70949277
% 112 -36.29349023
% 192 -36.98043419
% 342 -38.18509049
% 462 -38.99414085
% 1632 -44.91768959
% 3312 -46.00646639
% 6912 -47.26654005
% 14400 -47.6417499
% };
% % RVTDNN-2, line
% \addplot [color=mycolor2, dashdotted, line width=2.0pt]
% table {%
% 48 -35.70949277
% 112 -36.29349023
% 192 -36.98043419
% 342 -38.18509049
% 462 -38.99414085
% 1632 -44.91768959
% 3312 -46.00646639
% 6912 -47.26654005
% 14400 -47.6417499
% };
% \addlegendentry{$K=4$, RVTDNN~\cite{liu2004dynamic}}

% % R2TDNN-2, markers
% \addplot [color=mycolor3, mark=square, line width=2.0pt, only marks, mark options={solid, scale=1.25}, forget plot]
% table {%
% 50 -35.64754172
% 114 -37.65342158
% 194 -38.9177817
% 344 -40.06660531
% 464 -41.2428941
% 1634 -45.9260887
% 3314 -47.56770021
% 6914 -48.04333652
% 14402 -48.41244835
% };
% % R2TDNN-2, line
% \addplot [color=mycolor3, dashdotted, line width=2.0pt]
% table {%
% 50 -35.64754172
% 114 -37.65342158
% 194 -38.9177817
% 344 -40.06660531
% 464 -41.2428941
% 1634 -45.9260887
% 3314 -47.56770021
% 6914 -48.04333652
% 14402 -48.41244835
% };
% \addlegendentry{$K=4$, R2TDNN}

% RVTDNN-3, markers
\addplot [color=mycolor2, mark=square, line width=2.0pt,  only marks, mark options={solid, scale=1.25}, forget plot]
table {%
56 -35.5860029315701
96 -35.9386266023102
200 -36.6094267762085
504 -40.0268592329339
816 -42.3789268493807
1656 -45.0187081188689
3456 -46.6569516320603
7200 -47.723612452508
14616 -48.11296445773
};
\addplot [color=mycolor2, solid, line width=2.0pt]
table {%
56 -35.5860029315701
96 -35.9386266023102
200 -36.6094267762085
504 -40.0268592329339
816 -42.3789268493807
1656 -45.0187081188689
3456 -46.6569516320603
7200 -47.723612452508
14616 -48.11296445773
};
\addlegendentry{$K=5$, RVTDNN~\cite{liu2004dynamic}}

% ARVTDNN-3, markers
\addplot [color=mycolor4, mark=triangle, line width=2.0pt,  only marks, mark options={solid, scale=1.25}, forget plot]
table {%
104 -35.74396168814225
 168 -35.798241620770284
 320  -37.6438950760951
 720 -39.50826286874865
 1104  -41.426432274004405
 2088 -44.43348636222859
 4104 -46.89484396481982
 8160 -47.95745697553042
16008 -48.148945027637534
};
% ARVTDNN-3, line
\addplot [color=mycolor4, solid, line width=2.0pt]
table {%
104 -35.74396168814225
 168 -35.798241620770284
 320  -37.6438950760951
 720 -39.50826286874865
 1104  -41.426432274004405
 2088 -44.43348636222859
 4104 -46.89484396481982
 8160 -47.95745697553042
16008 -48.148945027637534
};
\addlegendentry{$K=5$, ARVTDNN~\cite{wang2018augmented}}

% R2TDNN-3, markers
\addplot [color=mycolor3, mark=x, line width=2.0pt,  only marks, mark options={solid, scale=1.75}, forget plot]
table {%
58 -35.6345385087577
98 -36.4898693553127
202 -38.9593260716023
506 -42.45566059712752
818 -43.8234926520851
1658 -45.9249481493807
3458 -47.4653743653488
7202 -48.4275162466823
14618 -48.4769841103719
};
% R2TDNN-3, line
\addplot [color=mycolor3, solid, line width=2.0pt]
table {%
58 -35.6345385087577
98 -36.4898693553127
202 -38.9593260716023
506 -42.45566059712752
818 -43.8234926520851
1658 -45.9249481493807
3458 -47.4653743653488
7202 -48.4275162466823
14618 -48.4769841103719
};
\addlegendentry{$K=5$, R2TDNN}

% Lower bound
\addplot [thick, black, dashed, line width=2.0pt]
table {%
24.324160830347 -50.1
15000 -50.1
};
\addlegendentry{Lower bound simulation}

\end{axis}

\end{tikzpicture}

==> Figures/loss_compare_1.tex <==
% \documentclass[tikz]{standalone}
% \usepackage[T1]{fontenc}
% \usepackage[utf8]{inputenc}
% \usepackage{pgfplots}
% \usepackage{grffile}
% \pgfplotsset{compat=newest}
% \usetikzlibrary{plotmarks}
% \usetikzlibrary{arrows.meta}
% \usepgfplotslibrary{patchplots}
% \usepackage{amsmath}

% \begin{document}

%
\begin{tikzpicture}[scale=\linewidth/14.8cm]
\definecolor{mycolor1}{rgb}{0.12156862745098039, 0.4666666666666667, 0.7058823529411765}%
\definecolor{mycolor2}{rgb}{1.0, 0.4980392156862745, 0.054901960784313725}%
\definecolor{mycolor3}{rgb}{0.17254901960784313, 0.6274509803921569, 0.17254901960784313}%
\definecolor{mycolor4}{rgb}{0.8392156862745098, 0.15294117647058825, 0.1568627450980392}%
\definecolor{mycolor5}{rgb}{0.5803921568627451, 0.403921568627451, 0.7411764705882353}%
\definecolor{mycolor6}{rgb}{0.5490196078431373, 0.33725490196078434, 0.29411764705882354}%
\definecolor{mycolor7}{rgb}{0.8901960784313725, 0.4666666666666667, 0.7607843137254902}%
\definecolor{mycolor8}{rgb}{0.4980392156862745, 0.4980392156862745, 0.4980392156862745}%
\definecolor{mycolor9}{rgb}{0.7372549019607844, 0.7411764705882353, 0.13333333333333333}%
\definecolor{mycolor10}{rgb}{0.09019607843137255, 0.7450980392156863, 0.8117647058823529}%

\begin{axis}[
width=12cm,
height=4cm,
at={(2.19in,0.9in)},
scale only axis,
legend cell align={left},
legend style={at={(1,1)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmajorgrids,
xmin=0, xmax=100,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={MSE},
ymajorgrids,
ymin=1e-05, ymax=1e-03,
yminorgrids,
ymode=log,
ytick style={color=black}
]
\addplot [mycolor2, dashed, line width=2.5pt]
table {%
0 0.0160356499254704
1 0.000437958427937701
2 0.000176822126377374
3 0.000137170194648206
4 0.000118155097879935
5 0.000105691477074288
6 9.66247462201864e-05
7 8.85981426108629e-05
8 8.24628878035583e-05
9 7.90255216998048e-05
10 7.71751438151114e-05
11 7.46862569940276e-05
12 7.29312523617409e-05
13 7.17585426173173e-05
14 6.96044517098926e-05
15 6.79342192597687e-05
16 6.6036700445693e-05
17 6.51887676212937e-05
18 6.40870493953116e-05
19 6.33317977190018e-05
20 6.28688794677146e-05
21 6.17922996752895e-05
22 6.11479044891894e-05
23 6.07200636295602e-05
24 6.00255589233711e-05
25 5.98840670136269e-05
26 5.94696939515416e-05
27 5.92580800002906e-05
28 5.84585577598773e-05
29 5.82532084081322e-05
30 5.77319842705037e-05
31 5.72633944102563e-05
32 5.72410099266563e-05
33 5.67761999263894e-05
34 5.63129251531791e-05
35 5.60387306904886e-05
36 5.57425992155913e-05
37 5.53820354980417e-05
38 5.49413380213082e-05
39 5.46106020919979e-05
40 5.44682698091492e-05
41 5.40937362529803e-05
42 5.41655754204839e-05
43 5.36238658241928e-05
44 5.35139770363458e-05
45 5.30204342794605e-05
46 5.26003932463937e-05
47 5.24947099620476e-05
48 5.24672032042872e-05
49 5.23136513947975e-05
50 5.20167195645627e-05
51 5.18085835210513e-05
52 5.16068394063041e-05
53 5.15204264956992e-05
54 5.12143233208917e-05
55 5.08973498654086e-05
56 5.01837093906943e-05
57 4.98649642395321e-05
58 4.94696978421416e-05
59 4.86609424115159e-05
60 4.85860509797931e-05
61 4.8402162065031e-05
62 4.83873882330954e-05
63 4.79119844385423e-05
64 4.76672903459985e-05
65 4.6377466787817e-05
66 4.55298541055527e-05
67 4.50148472737055e-05
68 4.5136795961298e-05
69 4.48831196990795e-05
70 4.45474579464644e-05
71 4.4342850742396e-05
72 4.44021461589728e-05
73 4.45036930614151e-05
74 4.42665586888324e-05
75 4.39612485934049e-05
76 4.38884380855598e-05
77 4.37542585132178e-05
78 4.40964868175797e-05
79 4.38829410995822e-05
80 4.42212622147053e-05
81 4.36851732956711e-05
82 4.34591311204713e-05
83 4.36067457485478e-05
84 4.31301014032215e-05
85 4.32178167102393e-05
86 4.30376567237545e-05
87 4.27878148911987e-05
88 4.27908671554178e-05
89 4.30479594797362e-05
90 4.2587133066263e-05
91 4.27735067205504e-05
92 4.26840815634932e-05
93 4.25787729909644e-05
94 4.27075901825447e-05
95 4.26762962888461e-05
96 4.25886100856587e-05
97 4.25782818638254e-05
98 4.27162522100843e-05
99 4.23363162553869e-05
100 4.24933386966586e-05
101 4.2322189983679e-05
102 4.21654876845423e-05
103 4.23450146627147e-05
104 4.22010343754664e-05
105 4.22496232204139e-05
106 4.23980709456373e-05
107 4.22923840233125e-05
108 4.19273310399149e-05
109 4.22000521211885e-05
110 4.20586875407025e-05
111 4.19002608396113e-05
112 4.24165336880833e-05
113 4.19287971453741e-05
114 4.19309508288279e-05
115 4.20487922383472e-05
116 4.16865077568218e-05
117 4.20940086769406e-05
118 4.16657239838969e-05
119 4.19047501054592e-05
120 4.19286552642006e-05
121 4.16022230638191e-05
122 4.14862697653007e-05
123 4.14457244914956e-05
124 4.18264644395094e-05
125 4.16684270021506e-05
126 4.1513703763485e-05
127 4.15958202211186e-05
128 4.16809234593529e-05
129 4.17476294387598e-05
130 4.14255264331587e-05
131 4.17770097556058e-05
132 4.14100395573769e-05
133 4.1364739445271e-05
134 4.15421309298836e-05
135 4.13561901950743e-05
136 4.14650166931096e-05
137 4.12876906921156e-05
138 4.12657209380995e-05
139 4.1099945519818e-05
140 4.13388479501009e-05
141 4.15696231357288e-05
142 4.12384870287497e-05
143 4.12673834944144e-05
144 4.09123858844396e-05
145 4.11411056120414e-05
146 4.09713757107966e-05
147 4.11950895795599e-05
148 4.08498563047033e-05
149 4.11086730309762e-05
150 4.10427674069069e-05
151 4.09177446272224e-05
152 4.07734005420934e-05
153 4.07712577725761e-05
154 4.11656073993072e-05
155 4.09276981372386e-05
156 4.08858759328723e-05
157 4.07823645218741e-05
158 4.06755498261191e-05
159 4.07041588914581e-05
160 4.06571052735671e-05
161 4.07529769290704e-05
162 4.06198487326037e-05
163 4.06055587518495e-05
164 4.064852691954e-05
165 4.06666767958086e-05
166 4.06454892072361e-05
167 4.0453585825162e-05
168 4.06229301006533e-05
169 4.05514183512423e-05
170 4.03584308514837e-05
171 4.02950245188549e-05
172 4.03052472393028e-05
173 4.03928388550412e-05
174 4.01550787501037e-05
175 4.03966841986403e-05
176 4.049360359204e-05
177 4.0160353819374e-05
178 4.0377679397352e-05
179 4.03394697059412e-05
180 4.02652767661493e-05
181 3.99849814129993e-05
182 4.00655626435764e-05
183 4.02461773774121e-05
184 4.0006165363593e-05
185 3.97948388126679e-05
186 3.9985949115362e-05
187 4.0054557757685e-05
188 4.02617661166005e-05
189 3.99794407712761e-05
190 3.99927230319008e-05
191 4.01290526497178e-05
192 3.97315307054669e-05
193 3.9677855966147e-05
194 3.95950228266884e-05
195 3.98305492126383e-05
196 3.99743039452005e-05
197 3.95799579564482e-05
198 3.96567702409811e-05
199 3.96077884943224e-05
};
\addlegendentry{$K=5$, RVTDNN~\cite{liu2004dynamic} Training}



\addplot[dotted, mycolor4, line width=2.5pt]
table{
0 0.00610089441761374
1 0.000278900726698339
2 0.000157957983901724
3 0.000119367206934839
4 0.000102282087027561
5 9.36059732339345e-05
6 8.79512590472586e-05
7 8.42246954562142e-05
8 8.00098132458515e-05
9 7.6730408181902e-05
10 7.3458366387058e-05
11 7.15877977199852e-05
12 6.94011978339404e-05
13 6.77340503898449e-05
14 6.65945917717181e-05
15 6.55907497275621e-05
16 6.40729485894553e-05
17 6.29740534350276e-05
18 6.25433676759712e-05
19 6.13791708019562e-05
20 6.09934686508495e-05
21 6.01224419369828e-05
22 5.93701297475491e-05
23 5.90231720707379e-05
24 5.82476459385362e-05
25 5.8255078329239e-05
26 5.71462478546891e-05
27 5.68952491448727e-05
28 5.67177994525991e-05
29 5.6298387789866e-05
30 5.62382119824179e-05
31 5.5726537539158e-05
32 5.57722232770175e-05
33 5.53266472707037e-05
34 5.53070749447215e-05
35 5.45882758160587e-05
36 5.45533039257862e-05
37 5.42057605343871e-05
38 5.38540698471479e-05
39 5.37147643626668e-05
40 5.34005484951194e-05
41 5.36853003723081e-05
42 5.31044970557559e-05
43 5.29821918462403e-05
44 5.26694893778767e-05
45 5.29322132933885e-05
46 5.29711396666244e-05
47 5.19218228873797e-05
48 5.22888403793331e-05
49 5.19362874911167e-05
50 5.17658118042164e-05
51 5.13964805577416e-05
52 5.16997934028041e-05
53 5.12622900714632e-05
54 5.13394297740888e-05
55 5.14393323101103e-05
56 5.09547280671541e-05
57 5.08708326378837e-05
58 5.12145743414294e-05
59 5.0980339437956e-05
60 5.07944969285745e-05
61 5.07643126184121e-05
62 5.04648669448216e-05
63 5.05202151543926e-05
64 5.04538911627606e-05
65 5.02665934618562e-05
66 5.00800342706498e-05
67 5.03072915307712e-05
68 4.99192465213127e-05
69 5.00344649481121e-05
70 5.01370413985569e-05
71 5.01643298775889e-05
72 4.97580149385612e-05
73 5.02206312376074e-05
74 4.96084940095898e-05
75 4.97617875225842e-05
76 4.97712717333343e-05
77 4.93193256261293e-05
78 4.93150291731581e-05
79 4.95013664476573e-05
80 4.94582491228357e-05
81 4.92120161652565e-05
82 4.93149163958151e-05
83 4.89988742629066e-05
84 4.92759827466216e-05
85 4.90947022626642e-05
86 4.88893456349615e-05
87 4.90136299049482e-05
88 4.90980200993363e-05
89 4.86402786918916e-05
90 4.87213037558831e-05
91 4.88247133034747e-05
92 4.84505544591229e-05
93 4.84489646623842e-05
94 4.844638533541e-05
95 4.86233220726717e-05
96 4.84371594211552e-05
97 4.83629191876389e-05
98 4.81101633340586e-05
99 4.85063137602992e-05
100 4.84751799376681e-05
101 4.82045579701662e-05
102 4.80940034321975e-05
103 4.81478091387544e-05
104 4.78903566545341e-05
105 4.80230264656711e-05
106 4.79453156003729e-05
107 4.77890898764599e-05
108 4.76290806545876e-05
109 4.77545363537502e-05
110 4.76608220196795e-05
111 4.83137446281034e-05
112 4.80155686091166e-05
113 4.76320492452942e-05
114 4.74050684715621e-05
115 4.75343331345357e-05
116 4.73529798910022e-05
117 4.73396248708013e-05
118 4.7265875764424e-05
119 4.73565305583179e-05
120 4.72757856186945e-05
121 4.71571802336257e-05
122 4.68220059701707e-05
123 4.72647079732269e-05
124 4.72005740448367e-05
125 4.69990409328602e-05
126 4.68030120828189e-05
127 4.69406295451336e-05
128 4.64990334876347e-05
129 4.65195116703399e-05
130 4.6685388952028e-05
131 4.68884099973366e-05
132 4.66383607999887e-05
133 4.62773205072153e-05
134 4.61388044641353e-05
135 4.62568496004678e-05
136 4.63839642179664e-05
137 4.6051645767875e-05
138 4.58512768091168e-05
139 4.59961847809609e-05
140 4.54436340078246e-05
141 4.51884152425919e-05
142 4.47694583272096e-05
143 4.4782198528992e-05
144 4.43971475760918e-05
145 4.46642734459601e-05
146 4.42929704149719e-05
147 4.43604985775892e-05
148 4.35233814641833e-05
149 4.36680566053838e-05
150 4.36168738815468e-05
151 4.34395296906587e-05
152 4.35519286838826e-05
153 4.31611151725519e-05
154 4.31555963587016e-05
155 4.29597384936642e-05
156 4.30428372055758e-05
157 4.31888729508501e-05
158 4.3047039071098e-05
159 4.27743980253581e-05
160 4.281004294171e-05
161 4.28664425271563e-05
162 4.30497821071185e-05
163 4.2845742427744e-05
164 4.25266807724256e-05
165 4.26690094172955e-05
166 4.27901177317835e-05
167 4.23020283051301e-05
168 4.26279329985846e-05
169 4.25760044890922e-05
170 4.24147729063407e-05
171 4.21625918534119e-05
172 4.21965269197244e-05
173 4.22565026383381e-05
174 4.19390162278432e-05
175 4.1828905523289e-05
176 4.22485209128354e-05
177 4.20302276324946e-05
178 4.21235999965575e-05
179 4.18976414948702e-05
180 4.18169329350349e-05
181 4.19502539443783e-05
182 4.16660732298624e-05
183 4.20018441218417e-05
184 4.17457922594622e-05
185 4.12817171309143e-05
186 4.15286631323397e-05
187 4.14340356655885e-05
188 4.15102040278725e-05
189 4.16918846894987e-05
190 4.13442649005447e-05
191 4.1387331293663e-05
192 4.13785783166531e-05
193 4.13670641137287e-05
194 4.10232241847552e-05
195 4.1410527046537e-05
196 4.15809990954585e-05
197 4.11661167163402e-05
198 4.09996864618734e-05
199 4.15019021602347e-05
};
\addlegendentry{$K=5$, ARVTDNN~\cite{wang2018augmented} Training}



\addplot [mycolor3, dashed, line width=2.5pt]
table {%
0 0.000296835525659844
1 0.000100608718639705
2 7.84515214036219e-05
3 6.39957434032112e-05
4 5.6942011724459e-05
5 5.19508685101755e-05
6 4.84336305817124e-05
7 4.604312198353e-05
8 4.46576596004888e-05
9 4.34739522461314e-05
10 4.16600414610002e-05
11 3.91589164792094e-05
12 3.68731489288621e-05
13 3.53259383700788e-05
14 3.41806116921362e-05
15 3.3514472306706e-05
16 3.28728783642873e-05
17 3.24134271068033e-05
18 3.20104663842358e-05
19 3.1614166800864e-05
20 3.13359960273374e-05
21 3.08578491967637e-05
22 3.05960056721233e-05
23 3.02910084428731e-05
24 2.99655275739497e-05
25 2.95661793643376e-05
26 2.93394641630584e-05
27 2.9050530429231e-05
28 2.87978728010785e-05
29 2.85676578641869e-05
30 2.8513919460238e-05
31 2.83164135908009e-05
32 2.80540552921593e-05
33 2.78973147942452e-05
34 2.76812716037966e-05
35 2.76056107395561e-05
36 2.74145277217031e-05
37 2.72450306511018e-05
38 2.71100634563481e-05
39 2.68783987849019e-05
40 2.67995837930357e-05
41 2.66321931121638e-05
42 2.65018206846435e-05
43 2.64201116806362e-05
44 2.62661651504459e-05
45 2.62770554400049e-05
46 2.61869881796883e-05
47 2.60742053797003e-05
48 2.59576427197317e-05
49 2.59642129094573e-05
50 2.57828978647012e-05
51 2.57710198638961e-05
52 2.5699291654746e-05
53 2.57631327258423e-05
54 2.56475505011622e-05
55 2.55551385635044e-05
56 2.54188544204226e-05
57 2.54954738920787e-05
58 2.54703336395323e-05
59 2.53663893090561e-05
60 2.53242960752686e-05
61 2.52829922828823e-05
62 2.52852169069229e-05
63 2.52341105806408e-05
64 2.51753863267368e-05
65 2.51806304731872e-05
66 2.51700330409221e-05
67 2.50606954068644e-05
68 2.50187604251551e-05
69 2.50832217716379e-05
70 2.49807380896527e-05
71 2.49452714342624e-05
72 2.47934349317802e-05
73 2.48522701440379e-05
74 2.48857941187453e-05
75 2.47365187533433e-05
76 2.47474854404572e-05
77 2.4691677026567e-05
78 2.46235867962241e-05
79 2.45925748458831e-05
80 2.45952505792957e-05
81 2.45481678575743e-05
82 2.44796628976474e-05
83 2.4477330953232e-05
84 2.43557024077745e-05
85 2.44302354985848e-05
86 2.42774349317187e-05
87 2.4313685571542e-05
88 2.42217010963941e-05
89 2.41507714235922e-05
90 2.41308935073903e-05
91 2.41260495386086e-05
92 2.40937224589288e-05
93 2.40466506511439e-05
94 2.40025838138536e-05
95 2.40433346334612e-05
96 2.39266719290754e-05
97 2.3788888938725e-05
98 2.38931952480925e-05
99 2.3824002710171e-05
100 2.37473668676103e-05
101 2.37112253671512e-05
102 2.36707692238269e-05
103 2.35820371017326e-05
104 2.35061888815835e-05
105 2.33893661061302e-05
106 2.34088493016316e-05
107 2.32897182286251e-05
108 2.33443734032335e-05
109 2.33147329709027e-05
110 2.32921211136272e-05
111 2.3231466911966e-05
112 2.31604954024078e-05
113 2.31797876040218e-05
114 2.31857466133079e-05
115 2.30831919907359e-05
116 2.3035083358991e-05
117 2.30547084356658e-05
118 2.29872512136353e-05
119 2.30330078920815e-05
120 2.29326087719528e-05
121 2.30770820053294e-05
122 2.30082750931615e-05
123 2.28113312914502e-05
124 2.28690441872459e-05
125 2.28990047617117e-05
126 2.28000062634237e-05
127 2.28089356824057e-05
128 2.28375429287553e-05
129 2.27987529797247e-05
130 2.2818303477834e-05
131 2.27335185627453e-05
132 2.28086337301647e-05
133 2.27339241973823e-05
134 2.27908240049146e-05
135 2.26872361963615e-05
136 2.26315787585918e-05
137 2.27155287575442e-05
138 2.26824231503997e-05
139 2.26430947805056e-05
140 2.26150114031043e-05
141 2.2672629711451e-05
142 2.2665228243568e-05
143 2.26265146920923e-05
144 2.25874136958737e-05
145 2.26295251195552e-05
146 2.25935964408563e-05
147 2.24865198106272e-05
148 2.26227421080694e-05
149 2.24846226046793e-05
150 2.24552150029922e-05
151 2.24983486987185e-05
152 2.24606174015207e-05
153 2.23559600271983e-05
154 2.23305378312944e-05
155 2.2318559786072e-05
156 2.22842500079423e-05
157 2.22428370761918e-05
158 2.23854967771331e-05
159 2.22358685277868e-05
160 2.21823665924603e-05
161 2.22484031837666e-05
162 2.21171903831419e-05
163 2.21619520743843e-05
164 2.21219743252732e-05
165 2.22024791582953e-05
166 2.21154296013992e-05
167 2.20842484850436e-05
168 2.20182901102817e-05
169 2.20703404920641e-05
170 2.20601086766692e-05
171 2.20384972635657e-05
172 2.21152458834695e-05
173 2.19430858123815e-05
174 2.19988614844624e-05
175 2.19584308069898e-05
176 2.19728171941824e-05
177 2.18957229662919e-05
178 2.19346566154854e-05
179 2.19383036892395e-05
180 2.17919787246501e-05
181 2.18068526010029e-05
182 2.18706718442263e-05
183 2.17820670513902e-05
184 2.17809501918964e-05
185 2.17377128137741e-05
186 2.16996832023142e-05
187 2.1789643142256e-05
188 2.17294000321999e-05
189 2.17493616219144e-05
190 2.17014985537389e-05
191 2.16497628571233e-05
192 2.16250609810231e-05
193 2.16542885027593e-05
194 2.17461438296596e-05
195 2.16173721128143e-05
196 2.1571033357759e-05
197 2.16177759284619e-05
198 2.16659846046241e-05
199 2.15813706745394e-05
};
\addlegendentry{$K=5$, R2TDNN Training}
\end{axis}
\end{tikzpicture}
% \end{document}


==> Figures/loss_compare_2.tex <==
% \documentclass[tikz]{standalone}
% \usepackage[T1]{fontenc}
% \usepackage[utf8]{inputenc}
% \usepackage{pgfplots}
% \usepackage{grffile}
% \pgfplotsset{compat=newest}
% \usetikzlibrary{plotmarks}
% \usetikzlibrary{arrows.meta}
% \usepgfplotslibrary{patchplots}
% \usepackage{amsmath}

% \begin{document}

%
\begin{tikzpicture}[scale=\linewidth/14.8cm]
\definecolor{mycolor1}{rgb}{0.12156862745098039, 0.4666666666666667, 0.7058823529411765}%
\definecolor{mycolor2}{rgb}{1.0, 0.4980392156862745, 0.054901960784313725}%
\definecolor{mycolor3}{rgb}{0.17254901960784313, 0.6274509803921569, 0.17254901960784313}%
\definecolor{mycolor4}{rgb}{0.8392156862745098, 0.15294117647058825, 0.1568627450980392}%
\definecolor{mycolor5}{rgb}{0.5803921568627451, 0.403921568627451, 0.7411764705882353}%
\definecolor{mycolor6}{rgb}{0.5490196078431373, 0.33725490196078434, 0.29411764705882354}%
\definecolor{mycolor7}{rgb}{0.8901960784313725, 0.4666666666666667, 0.7607843137254902}%
\definecolor{mycolor8}{rgb}{0.4980392156862745, 0.4980392156862745, 0.4980392156862745}%
\definecolor{mycolor9}{rgb}{0.7372549019607844, 0.7411764705882353, 0.13333333333333333}%
\definecolor{mycolor10}{rgb}{0.09019607843137255, 0.7450980392156863, 0.8117647058823529}%

\begin{axis}[
width=12cm,
height=4cm,
at={(2.19in,0.9in)},
scale only axis,
legend cell align={left},
legend style={at={(1,1)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmajorgrids,
xmin=0, xmax=100,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={MSE},
ymajorgrids,
ymin=1e-05, ymax=1e-03,
yminorgrids,
ymode=log,
ytick style={color=black}
]

\addplot [solid, mycolor2, line width=2.0pt]
table {%
0 0.00108900608029217
1 0.00022411861573346
2 0.000155902380356565
3 0.000128698578919284
4 0.000112269422970712
5 0.000103597594716121
6 9.24759515328333e-05
7 8.61116204760037e-05
8 8.14017621451057e-05
9 7.95667438069358e-05
10 7.62189010856673e-05
11 7.34066634322517e-05
12 7.41781914257444e-05
13 7.07804647390731e-05
14 6.93736947141588e-05
15 6.6893313487526e-05
16 6.5784523030743e-05
17 6.36659024166875e-05
18 6.42026134300977e-05
19 6.44485699012876e-05
20 6.14032178418711e-05
21 6.11563518759795e-05
22 6.13813535892405e-05
23 6.24204913037829e-05
24 5.92065043747425e-05
25 6.16606703260913e-05
26 5.9983129176544e-05
27 5.89188566664234e-05
28 5.74078367208131e-05
29 5.78354847675655e-05
30 5.73780489503406e-05
31 5.65780756005552e-05
32 5.79812221985776e-05
33 5.59732325200457e-05
34 5.57299026695546e-05
35 5.6142143876059e-05
36 5.47511590411887e-05
37 5.4643092880724e-05
38 5.44277318113018e-05
39 5.43753158126492e-05
40 5.42772068001796e-05
41 5.30536890437361e-05
42 5.25341383763589e-05
43 5.29592325619888e-05
44 5.3437048336491e-05
45 5.3659183322452e-05
46 5.17112239322159e-05
47 5.19548520969693e-05
48 5.25653886143118e-05
49 5.28201235283632e-05
50 5.23694216099102e-05
51 5.16528307343833e-05
52 5.15647770953365e-05
53 5.13737686560489e-05
54 5.19980385433882e-05
55 5.23512499057688e-05
56 5.21985821251292e-05
57 4.85556811327115e-05
58 4.84962001792155e-05
59 4.76925015391316e-05
60 4.76418754260521e-05
61 4.69681763206609e-05
62 5.11092657689005e-05
63 4.75280903629027e-05
64 4.56360576208681e-05
65 4.44717443315312e-05
66 4.61576419183984e-05
67 4.58641879959032e-05
68 4.49980252597015e-05
69 4.51876912848093e-05
70 4.33624045399483e-05
71 4.45656514784787e-05
72 4.34705034422223e-05
73 4.53892971563619e-05
74 4.67674944957253e-05
75 4.37123635492753e-05
76 4.45200348622166e-05
77 4.42565542471129e-05
78 4.44761717517395e-05
79 4.38872921222355e-05
80 4.40649819211103e-05
81 4.31151638622396e-05
82 4.38528513768688e-05
83 4.26719852839597e-05
84 4.29565370723139e-05
85 4.33857640018687e-05
86 4.30236941610929e-05
87 4.26416554546449e-05
88 4.23909696110059e-05
89 4.22839766542893e-05
90 4.29838255513459e-05
91 4.25921971327625e-05
92 4.21231961809099e-05
93 4.34793364547659e-05
94 4.29340143455192e-05
95 4.49154940724839e-05
96 4.16344773839228e-05
97 4.27926643169485e-05
98 4.19432217313442e-05
99 4.35547262895852e-05
100 4.20128817495424e-05
101 4.46978701802436e-05
102 4.20276701333933e-05
103 4.33913046435919e-05
104 4.33116947533563e-05
105 4.24535501224454e-05
106 4.21354634454474e-05
107 4.19119496655185e-05
108 4.41702468378935e-05
109 4.2196024878649e-05
110 4.24863828811795e-05
111 4.31600237789098e-05
112 4.27935847255867e-05
113 4.17757764807902e-05
114 4.1405510273762e-05
115 4.25954385718796e-05
116 4.1635077650426e-05
117 4.14967980759684e-05
118 4.22600787715055e-05
119 4.37736453022808e-05
120 4.1861323552439e-05
121 4.13412126363255e-05
122 4.16356706409715e-05
123 4.11926193919498e-05
124 4.09424173994921e-05
125 4.22791054006666e-05
126 4.41222000517882e-05
127 4.27114100602921e-05
128 4.13162451877724e-05
129 4.1660008719191e-05
130 4.19889111071825e-05
131 4.08395317208488e-05
132 4.11302498832811e-05
133 4.21411969000474e-05
134 4.09265048801899e-05
135 4.18419112975243e-05
136 4.08323649025988e-05
137 4.04421916755382e-05
138 4.28494204243179e-05
139 4.10284592362586e-05
140 4.19754578615539e-05
141 4.14064597862307e-05
142 4.02578116336372e-05
143 4.28970597567968e-05
144 4.08399682783056e-05
145 4.25313337473199e-05
146 4.11257497034967e-05
147 4.16869334003422e-05
148 4.00948629248887e-05
149 4.14804526371881e-05
150 4.10053871746641e-05
151 4.02621699322481e-05
152 4.00636345148087e-05
153 4.08382111345418e-05
154 4.11740184063092e-05
155 4.00578246626537e-05
156 4.11346554756165e-05
157 3.98439733544365e-05
158 4.03194862883538e-05
159 3.97957192035392e-05
160 4.16882794525009e-05
161 4.06113140343223e-05
162 3.99489254050422e-05
163 4.02296427637339e-05
164 4.24935788032599e-05
165 4.53001775895245e-05
166 4.11086257372517e-05
167 4.12309163948521e-05
168 4.00061617256142e-05
169 3.98471020162106e-05
170 3.95116730942391e-05
171 4.02650803152937e-05
172 3.9995491533773e-05
173 4.09859894716647e-05
174 4.07139996241312e-05
175 4.01009274355602e-05
176 4.04931670345832e-05
177 4.17959927290212e-05
178 3.99693199142348e-05
179 4.04624079237692e-05
180 4.01882316509727e-05
181 3.89239612559322e-05
182 3.8966001739027e-05
183 3.94435919588432e-05
184 3.88031112379394e-05
185 3.90223613067064e-05
186 4.10725042456761e-05
187 3.98574156861287e-05
188 4.07182778872084e-05
189 4.47167876700405e-05
190 4.17565352108795e-05
191 3.87191066693049e-05
192 4.00800890929531e-05
193 3.88174594263546e-05
194 3.86706124118064e-05
195 4.04430611524731e-05
196 3.86691426683683e-05
197 3.92615402233787e-05
198 3.85324965463951e-05
199 3.90858003811445e-05
};
\addlegendentry{$K=5$, RVTDNN~\cite{liu2004dynamic} Validation}


\addplot [solid, mycolor4, line width=2.0pt]
table {%
0 0.000503194576594979
1 0.000194121690583415
2 0.000135510126710869
3 0.000109597924165428
4 0.000101361656561494
5 9.29502712097019e-05
6 8.72879827511497e-05
7 8.07206524768844e-05
8 8.07147443993017e-05
9 7.62582931201905e-05
10 7.29759849491529e-05
11 7.04488847986795e-05
12 6.83324469719082e-05
13 6.78003780194558e-05
14 6.74987022648565e-05
15 7.42074553272687e-05
16 6.36675176792778e-05
17 6.29433779977262e-05
18 6.06118155701552e-05
19 6.204227975104e-05
20 6.30033100605942e-05
21 6.01690771873109e-05
22 5.87333306611981e-05
23 6.26070032012649e-05
24 5.70369847991969e-05
25 5.71163545828313e-05
26 5.81287677050568e-05
27 5.63433895877097e-05
28 5.77490682189818e-05
29 5.81529930059332e-05
30 5.58104293304496e-05
31 5.73910656385124e-05
32 5.52634046471212e-05
33 5.63716421311256e-05
34 5.51937228010502e-05
35 5.473236888065e-05
36 5.52410019736271e-05
37 5.74081714148633e-05
38 5.43314745300449e-05
39 5.48652460565791e-05
40 5.58867286599707e-05
41 5.50277218280826e-05
42 5.34103673999198e-05
43 5.30248835275415e-05
44 5.48639545741025e-05
45 5.47686395293567e-05
46 5.26131552760489e-05
47 5.22822374477983e-05
48 5.28931377630215e-05
49 5.41450608579908e-05
50 5.37472187716048e-05
51 5.19995373906568e-05
52 5.2601368224714e-05
53 5.13448067067657e-05
54 5.72695389564615e-05
55 5.49766118638217e-05
56 5.47346753592137e-05
57 5.43239657417871e-05
58 5.12111619173083e-05
59 5.26138828718103e-05
60 5.17129556101281e-05
61 5.11693287990056e-05
62 5.09409182996023e-05
63 5.08186712977476e-05
64 5.08186531078536e-05
65 5.01507747685537e-05
66 4.99790403409861e-05
67 5.11294201714918e-05
68 5.02798975503538e-05
69 5.00567657581996e-05
70 5.13261911692098e-05
71 5.19252462254371e-05
72 5.0550966989249e-05
73 5.10277641296852e-05
74 5.1356964831939e-05
75 5.28239834238775e-05
76 5.00037422170863e-05
77 5.21563815709669e-05
78 5.02039365528617e-05
79 4.999131851946e-05
80 5.20936664543115e-05
81 5.4569714848185e-05
82 5.53503814444412e-05
83 5.18119741172995e-05
84 4.92494145873934e-05
85 5.2651663281722e-05
86 4.97395412821788e-05
87 5.14238963660318e-05
88 5.08906596223824e-05
89 4.97655018989462e-05
90 4.91064674861263e-05
91 5.15102910867427e-05
92 4.88939294882584e-05
93 5.10079553350806e-05
94 5.43966780242044e-05
95 4.86893040942959e-05
96 4.87404431623872e-05
97 4.92647268401925e-05
98 5.42000307177659e-05
99 4.93881489092018e-05
100 5.26723924849648e-05
101 4.96849788760301e-05
102 5.14836319780443e-05
103 4.89003541588318e-05
104 4.82359682791866e-05
105 4.89230478706304e-05
106 4.81688366562594e-05
107 4.89351659780368e-05
108 4.97325563628692e-05
109 5.00446258229204e-05
110 4.88165205752011e-05
111 4.9436763220001e-05
112 4.83562362205703e-05
113 4.75633460155223e-05
114 4.79730624647345e-05
115 4.73099971713964e-05
116 4.79173286294099e-05
117 4.80364142276812e-05
118 4.82392570120282e-05
119 4.77890571346506e-05
120 4.7900863137329e-05
121 4.95645654154941e-05
122 4.78173606097698e-05
123 4.80012131447438e-05
124 4.91546925331932e-05
125 4.69858896394726e-05
126 4.90133461426012e-05
127 4.83734729641583e-05
128 4.78123984066769e-05
129 4.69218102807645e-05
130 4.62073840026278e-05
131 4.85428972751833e-05
132 4.70579325337894e-05
133 4.63179821963422e-05
134 4.65733683086e-05
135 4.57286878372543e-05
136 4.60655464848969e-05
137 4.80061098642182e-05
138 4.5652730477741e-05
139 4.65470402559731e-05
140 4.55689769296441e-05
141 4.54817891295534e-05
142 4.43438184447587e-05
143 4.45480181952007e-05
144 4.46172925876454e-05
145 5.17752050654963e-05
146 4.52288768428843e-05
147 4.48997125204187e-05
148 4.53271495644003e-05
149 4.40520670963451e-05
150 4.3076910515083e-05
151 4.3778563849628e-05
152 5.01232134411111e-05
153 4.32753367931582e-05
154 4.42148411821108e-05
155 4.32318884122651e-05
156 4.22709963459056e-05
157 4.27703671448398e-05
158 4.33404820796568e-05
159 4.27328632213175e-05
160 4.36861737398431e-05
161 4.45589357696008e-05
162 4.3950327381026e-05
163 4.79389236716088e-05
164 4.35661531810183e-05
165 4.29469655500725e-05
166 4.2179504816886e-05
167 4.17652590840589e-05
168 4.65733101009391e-05
169 4.22503217123449e-05
170 4.26933875132818e-05
171 4.33016684837639e-05
172 4.29267784056719e-05
173 4.45352925453335e-05
174 4.17518967879005e-05
175 4.16354523622431e-05
176 4.23513156420086e-05
177 4.35291185567621e-05
178 4.23017299908679e-05
179 4.49371145805344e-05
180 4.23031669924967e-05
181 4.22906305175275e-05
182 4.40497024101205e-05
183 4.30749460065272e-05
184 4.09558342653327e-05
185 4.21742515754886e-05
186 4.17328483308665e-05
187 4.24870049755555e-05
188 4.24436548200902e-05
189 4.25022408307996e-05
190 4.12906483688857e-05
191 4.27727864007466e-05
192 4.3130279664183e-05
193 4.27130216849037e-05
194 4.13325069530401e-05
195 4.31778280471917e-05
196 4.33379573223647e-05
197 4.07189945690334e-05
198 4.20503602072131e-05
199 4.08642226830125e-05
};
\addlegendentry{$K=5$, ARVTDNN~\cite{wang2018augmented} Validation}

\addplot [solid, mycolor3, line width=2.0pt]
table {%
0 0.000120369470096193
1 8.95663106348366e-05
2 7.02770994394086e-05
3 6.05971945333295e-05
4 5.55710030312184e-05
5 5.2413761295611e-05
6 4.88218902319204e-05
7 4.66864221380092e-05
8 4.52099848189391e-05
9 4.38131428381894e-05
10 4.13541274610907e-05
11 3.90723216696642e-05
12 3.71915448340587e-05
13 3.61116362910252e-05
14 3.41862069035415e-05
15 3.42734274454415e-05
16 3.31505652866326e-05
17 3.29010945279151e-05
18 3.27272282447666e-05
19 3.19935352308676e-05
20 3.19702012347989e-05
21 3.14145981974434e-05
22 3.09592942357995e-05
23 3.06262918456923e-05
24 3.04038621834479e-05
25 2.9703453037655e-05
26 2.93133325612871e-05
27 2.90672032861039e-05
28 2.84347825072473e-05
29 2.86938939098036e-05
30 2.83785338979214e-05
31 2.91855430987198e-05
32 2.77445287792943e-05
33 2.77400104096159e-05
34 2.80067379208049e-05
35 2.71355056611355e-05
36 2.74613521469291e-05
37 2.68733710981905e-05
38 2.67540090135299e-05
39 2.65504932031035e-05
40 2.66243096120888e-05
41 2.6727491786005e-05
42 2.64981117652496e-05
43 2.63891688518925e-05
44 2.66624119831249e-05
45 2.62540306721348e-05
46 2.59509615716524e-05
47 2.5712701244629e-05
48 2.60792530752951e-05
49 2.58175514318282e-05
50 2.54072965617524e-05
51 2.53130256169243e-05
52 2.55822887993418e-05
53 2.62583762378199e-05
54 2.55952600127785e-05
55 2.53591661021346e-05
56 2.58592954196502e-05
57 2.52777808782412e-05
58 2.49688418989535e-05
59 2.49948552664137e-05
60 2.54048791248351e-05
61 2.54676670010667e-05
62 2.54231308645103e-05
63 2.4727367417654e-05
64 2.46809559030226e-05
65 2.50099637923995e-05
66 2.50420889642555e-05
67 2.49822878686246e-05
68 2.47012339968933e-05
69 2.46796535066096e-05
70 2.48278993240092e-05
71 2.46403888013447e-05
72 2.44288276007865e-05
73 2.48097967414651e-05
74 2.43717222474515e-05
75 2.44300135818776e-05
76 2.44708589889342e-05
77 2.46692088694545e-05
78 2.46686122409301e-05
79 2.43334634433268e-05
80 2.51545006904053e-05
81 2.47493171627866e-05
82 2.44272487179842e-05
83 2.40977005887544e-05
84 2.40019835473504e-05
85 2.39684432017384e-05
86 2.41812867898261e-05
87 2.41456618823577e-05
88 2.38014945352916e-05
89 2.38703378272476e-05
90 2.37567492149537e-05
91 2.38032171182567e-05
92 2.46601484832354e-05
93 2.41351081058383e-05
94 2.42068508669036e-05
95 2.40507233684184e-05
96 2.37018430198077e-05
97 2.36760424741078e-05
98 2.45915125560714e-05
99 2.38174889091169e-05
100 2.39631972362986e-05
101 2.39049750234699e-05
102 2.38449047174072e-05
103 2.31141129916068e-05
104 2.36804880842101e-05
105 2.32490656344453e-05
106 2.34824310609838e-05
107 2.32299171329942e-05
108 2.32870352192549e-05
109 2.34457984333858e-05
110 2.31421818170929e-05
111 2.29518846026622e-05
112 2.34105064009782e-05
113 2.3189817511593e-05
114 2.29407869483111e-05
115 2.33457012654981e-05
116 2.28978806262603e-05
117 2.27563887165161e-05
118 2.29544275498483e-05
119 2.30626319535077e-05
120 2.3626487745787e-05
121 2.33100108744111e-05
122 2.28467124543386e-05
123 2.30446312343702e-05
124 2.29065663006622e-05
125 2.29484467126895e-05
126 2.2881828044774e-05
127 2.30378682317678e-05
128 2.30274818022735e-05
129 2.27087548410054e-05
130 2.33597002079478e-05
131 2.3363392756437e-05
132 2.27414475375554e-05
133 2.25037165364483e-05
134 2.30287296290044e-05
135 2.27053624257678e-05
136 2.263198075525e-05
137 2.27561013161903e-05
138 2.25243711611256e-05
139 2.29168781515909e-05
140 2.29047764150891e-05
141 2.28525004786206e-05
142 2.26219763135305e-05
143 2.26679276238428e-05
144 2.29949018830666e-05
145 2.25416315515758e-05
146 2.26032334467163e-05
147 2.29639736062381e-05
148 2.22239214053843e-05
149 2.25178046093788e-05
150 2.30487712542526e-05
151 2.24961095227627e-05
152 2.30258483497892e-05
153 2.24712821363937e-05
154 2.21405989577761e-05
155 2.23102761083283e-05
156 2.28072367463028e-05
157 2.23062434088206e-05
158 2.25644635065692e-05
159 2.29818779189372e-05
160 2.26328156713862e-05
161 2.23701208597049e-05
162 2.26728789129993e-05
163 2.33873724937439e-05
164 2.22313501581084e-05
165 2.24811919906642e-05
166 2.31192443607142e-05
167 2.23497190745547e-05
168 2.29473553190473e-05
169 2.20183028432075e-05
170 2.2380245354725e-05
171 2.30194928008132e-05
172 2.24057694140356e-05
173 2.22477174247615e-05
174 2.19077282963553e-05
175 2.19365156226559e-05
176 2.21066438825801e-05
177 2.2188058210304e-05
178 2.24354316742392e-05
179 2.23096139961854e-05
180 2.20617894228781e-05
181 2.23374263441656e-05
182 2.17672550206771e-05
183 2.27395648835227e-05
184 2.20033016375965e-05
185 2.20118872675812e-05
186 2.20351703319466e-05
187 2.19262383325258e-05
188 2.22044527617982e-05
189 2.19893536268501e-05
190 2.21230529859895e-05
191 2.19420635403367e-05
192 2.19526245928137e-05
193 2.20485526369885e-05
194 2.26756292249775e-05
195 2.21948139369488e-05
196 2.26540796575136e-05
197 2.20797501242487e-05
198 2.19720204768237e-05
199 2.20771125896135e-05
};
\addlegendentry{$K=5$, R2TDNN Validation}
\end{axis}
\end{tikzpicture}
% \end{document}


==> Figures/nmse_vs_flops.tex <==
% % This file was created by tikzplotlib v0.9.1.
% \documentclass[tikz]{standalone}
% \usepackage[T1]{fontenc}
% \usepackage[utf8]{inputenc}
% \usepackage{pgfplots}
% \usepackage{grffile}
% \pgfplotsset{compat=newest}
% \usetikzlibrary{plotmarks}
% \usetikzlibrary{arrows.meta}
% \usepgfplotslibrary{patchplots}
% \usepackage{amsmath}

% \begin{document}

\begin{tikzpicture}[scale=\linewidth/14cm]
\definecolor{mycolor1}{rgb}{0.12156862745098039, 0.4666666666666667, 0.7058823529411765}%
\definecolor{mycolor2}{rgb}{1.0, 0.4980392156862745, 0.054901960784313725}%
\definecolor{mycolor3}{rgb}{0.17254901960784313, 0.6274509803921569, 0.17254901960784313}%
\definecolor{mycolor4}{rgb}{0.8392156862745098, 0.15294117647058825, 0.1568627450980392}%
\definecolor{mycolor5}{rgb}{0.5803921568627451, 0.403921568627451, 0.7411764705882353}%
\definecolor{mycolor6}{rgb}{0.5490196078431373, 0.33725490196078434, 0.29411764705882354}%
\definecolor{mycolor7}{rgb}{0.8901960784313725, 0.4666666666666667, 0.7607843137254902}%
\definecolor{mycolor8}{rgb}{0.4980392156862745, 0.4980392156862745, 0.4980392156862745}%
\definecolor{mycolor9}{rgb}{0.7372549019607844, 0.7411764705882353, 0.13333333333333333}%
\definecolor{mycolor10}{rgb}{0.09019607843137255, 0.7450980392156863, 0.8117647058823529}%

\begin{axis}[%
width=12cm,
height=9cm,
at={(2.19in,0.9in)},
scale only axis,
legend cell align={left},
legend style={at={(1,1)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black},
log basis x={10},
tick align=outside,
tick pos=left,
 grid style={white!69.0196078431373!black},
xlabel style={font=\color{white!15!black}},
xlabel={Number of FLOPs},
xmajorgrids,
xmin=44, xmax=16008,
xminorgrids,
xmode=log,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel style={font=\color{white!15!black}},
ylabel={NMSE (dB)},
ymajorgrids,
ymin=-41, ymax=-26,
yminorgrids,
ytick style={color=black}
]
% GMP-markers
\addplot [color=mycolor1, only marks, line width=2.0pt, mark=o, mark options={solid, color=mycolor1, scale=1.25}, forget plot]
table{%
44 -27.4912375733462
62 -28.4423699435213
94 -31.2037946032652
188 -32.6573133541225
284 -33.2897687909
514 -33.3345706435582
744 -33.2238111517203
1916 -33.1484334372905
};
%GMP line
\addplot [color=mycolor1, solid, line width=2.0pt]
table{%
44 -27.4912375733462
62 -28.4423699435213
94 -31.2037946032652
188 -32.6573133541225
284 -33.2897687909
514 -33.3345706435582
744 -33.2238111517203
1916 -33.1484334372905
};
\addlegendentry{GMP~\cite{GMP_2006}}


% RVTDNN-1, markers
\addplot [color=mycolor2, only marks, line width=2.0pt, mark=square, mark options={solid, mycolor2, scale=1.25}, forget plot]
table {%
60 -27.4551736260765
100 -27.7560063006484
200 -28.5076979631594
440 -30.9163019893522
880 -33.1719040943119
1760 -35.2722372634919
3480 -36.813153090288
6980 -36.8048391224281
14000 -36.5818099484116
};
% RVTDNN-1 line
\addplot [color= mycolor2, dashed, line width=2.0pt]
table {%
60 -27.4551736260765
100 -27.7560063006484
200 -28.5076979631594
440 -30.9163019893522
880 -33.1719040943119
1760 -35.2722372634919
3480 -36.813153090288
6980 -36.8048391224281
14000 -36.5818099484116
};
\addlegendentry{$K=3$, RVTDNN~\cite{liu2004dynamic}}

\addplot [color=mycolor4, only marks, line width=2.0pt, mark=triangle, mark options={solid, mycolor4, scale=1.25}, forget plot]
table {%
132 -28.025303813965017
220 -29.02733009360863
440  -30.61705167053422
968  -31.86811226180662
1936  -34.104105665998595
3872 -35.92353822146018
7656 -36.87544611519037
15356 -36.95969841450626
};

\addplot[color=mycolor4, dashed, line width=2.0pt]
table{
132 -28.025303813965017
220 -29.02733009360863
440  -30.61705167053422
968  -31.86811226180662
1936  -34.104105665998595
3872 -35.92353822146018
7656 -36.87544611519037
15356 -36.95969841450626
%30800 -36.61863399153673
};
\addlegendentry{$K=3$, ARVTDNN~\cite{wang2018augmented}}


% R2TDNN-1, markers
\addplot [color=mycolor3, only marks, line width=2.0pt, mark=x, mark options={solid, mycolor3, scale = 1.75}, forget plot]
table {%
62 -27.46500185
102 -28.32238479
202 -29.00095478
522 -31.26343171
802 -33.7527232
1562 -35.45415675
3202 -36.73365619
6402 -36.92128142
13282 -37.16281201
};
% R2TDNN-1, line
\addplot [color=mycolor3, dashed, line width=2.0pt]
table {%
62 -27.46500185
102 -28.32238479
202 -29.00095478
522 -31.26343171
802 -33.7527232
1562 -35.45415675
3202 -36.73365619
6402 -36.92128142
13282 -37.16281201
};
\addlegendentry{$K=3$, R2TDNN}


% % RVTDNN-2, markers
% \addplot [color=mycolor2, mark=square,line width=2.0pt, only marks, mark options={solid, scale=1.25}, forget plot]
% table {%
% 48 -27.53674681
% 112 -27.78889011
% 192 -28.76634616
% 342 -29.68919031
% 462 -30.21081444
% 1632 -35.82453051
% 3312 -36.44080264
% 6912 -36.64260083
% 14400 -36.94920482
% };
% % RVTDNN-2, line
% \addplot [color=mycolor2, dashdotted, line width=2.0pt]
% table {%
% 48 -27.53674681
% 112 -27.78889011
% 192 -28.76634616
% 342 -29.68919031
% 462 -30.21081444
% 1632 -35.82453051
% 3312 -36.44080264
% 6912 -36.64260083
% 14400 -36.94920482
% };
% \addlegendentry{$K=4$, RVTDNN~\cite{liu2004dynamic}}

% % R2TDNN-2, markers
% \addplot [color=mycolor3, mark=x, line width=2.0pt, only marks, mark options={solid, scale=1.75}, forget plot]
% table {%
% 50 -27.55587556
% 114 -28.87141951
% 194 -30.51861984
% 344 -31.49562006
% 464 -32.58717058
% 1634 -36.58446276
% 3314 -37.41813132
% 6914 -37.61928023
% 14402 -37.93478195
% };
% % R2TDNN-2, line
% \addplot [color=mycolor3, dashdotted, line width=2.0pt]
% table {%
% 50 -27.55587556
% 114 -28.87141951
% 194 -30.51861984
% 344 -31.49562006
% 464 -32.58717058
% 1634 -36.58446276
% 3314 -37.41813132
% 6914 -37.61928023
% 14402 -37.93478195
% };
% \addlegendentry{$K=4$, R2TDNN}

% RVTDNN-3, markers
\addplot [color=mycolor2, mark=square, line width=2.0pt,  only marks, mark options={solid, scale=1.25}, forget plot]
table {%
56 -27.4783363909303
96 -27.5721369269017
200 -28.2723704742848
504 -31.45355314436253
816 -34.0385526568819
1656 -36.1492055570726
3456 -36.5315038267091
7200 -37.4055703671491
14616 -37.168637884974
};
\addplot [color=mycolor2, solid, line width=2.0pt]
table {%
56 -27.4783363909303
96 -27.5721369269017
200 -28.2723704742848
504 -31.45355314436253
816 -34.0385526568819
1656 -36.1492055570726
3456 -36.5315038267091
7200 -37.4055703671491
14616 -37.168637884974
};
\addlegendentry{$K=5$, RVTDNN~\cite{liu2004dynamic}}

% ARVTDNN-3, markers
\addplot [color=mycolor4, mark=triangle, line width=2.0pt,  only marks, mark options={solid, scale=1.25}, forget plot]
table {%
104 -27.582168084025255
 168 -27.682335162177078
 320  -29.138918969714016
 720 -31.27016859445749
 1104  -32.84041479582547
 2088  -35.05976840922704
 4104 -36.905955371194105
 8160 -37.601123825845585
16008 -37.69438359510872
};
% ARVTDNN-3, line
\addplot [color=mycolor4, solid, line width=2.0pt]
table {%
104 -27.582168084025255
 168 -27.682335162177078
 320  -29.138918969714016
 720 -31.27016859445749
 1104  -32.84041479582547
 2088  -35.05976840922704
 4104 -36.905955371194105
 8160 -37.601123825845585
16008 -37.69438359510872
};
\addlegendentry{$K=5$, ARVTDNN~\cite{wang2018augmented}}

% R2TDNN-3, markers
\addplot [color=mycolor3, mark=x, line width=2.0pt,  only marks, mark options={solid, scale=1.75}, forget plot]
table {%
58 -27.5659921396353
98 -28.2125968212446
202 -30.4482396876335
506 -33.66894569608883
818 -35.2962880875222
1658 -36.6441225475589
3458 -37.499711810627
7202 -37.8704336693423
14618 -37.9554737473432
};
% R2TDNN-3, line
\addplot [color=mycolor3, solid, line width=2.0pt]
table {%
58 -27.5659921396353
98 -28.2125968212446
202 -30.4482396876335
506 -33.66894569608883
818 -35.2962880875222
1658 -36.6441225475589
3458 -37.499711810627
7202 -37.8704336693423
14618 -37.9554737473432
};
\addlegendentry{$K=5$, R2TDNN}

% Lower bound
\addplot [thick, color=black, line width=2.0pt]
table {%
24.324160830347 -40.17
16000 -40.17
};
\addlegendentry{Lower bound}

\end{axis}

\end{tikzpicture}
%

% \end{document}

